Argument Mining Driven Analysis of Peer-Reviews

Peer reviewing is a central process in modern research and essential for ensuring high quality and reliability of published work. At the same time, it is a time-consuming process and increasing interest in emerging fields often results in a high review workload, especially for senior researchers in this area. How to cope with this problem is an open question and it is vividly discussed across all major conferences. In this work, we propose an Argument Mining based approach for the assistance of editors, meta-reviewers, and reviewers. We demonstrate that the decision process in the field of scientific publications is driven by arguments and automatic argument identification is helpful in various use-cases. One of our findings is that arguments used in the peer-review process differ from arguments in other domains making the transfer of pre-trained models difficult. Therefore, we provide the community with a new peer-review dataset from different computer science conferences with annotated arguments. In our extensive empirical evaluation, we show that Argument Mining can be used to efficiently extract the most relevant parts from reviews, which are paramount for the publication decision. The process remains interpretable since the extracted arguments can be highlighted in a review without detaching them from their context.

==> review_examples/midl19_52_2.tex <==
This paper proposes to use a CNN architecture to reconstruct MR Fingerprinting parametric maps.  The authors test their algorithm on a dataset of 95 subjects for neuromuscular disease. They compare their method with two state of the art deep learning methods and illustrate superior performance on NRMSE, PSNR, SSIM and R2 metrics. Moreover, they have done some ablation studies to show the importance of the receptive field and temporal frames for MRF reconstruction.

\textcolor{green}{I believe the experiments are thorough and well designed to back the claims of the paper.} \textcolor{red}{The utilized network architecture can be better explained with an emphasis on specific design choices.}

1- \textcolor{green}{This paper is well written and the message is clear to the reader.} 
2- \textcolor{green}{The extensive tests on a real dataset instead of phantom cases is definitely a strength of the paper.}    

3- The description of the network architecture is not clear for the reader. How does the temporal and spatial blocks work? They seem to work in different dimensions of the signals. Even though the authors explain the details in the text I believe an additional illustration in each block (maybe in Appendix) might be helpful to reproduce the method in the paper for further research.
4- How does the specifics of the network architecture influence the performance? Why do the authors reuse  the input of a temporal block to its output and how does this influence the performance?
5- How is the complex component of the signal concatenated into a channel ? Does the order of concatenation influence the results? Did the authors considered to utilize complex valued networks for this task? 
6- The quantitative results are yielded using multiple segmentation masks due to MR physics related concerns. Are the results on Table 1 heavily dependent on use of these masks? Are the results on the entire parametric maps in line with the current results?    
7- What is the number of parameters required for each method in Table 1? The reason for high performance of the proposed method can be explained with the required number of parameters to train the method. Please elaborate on this.
8-The lack of scalability and the requirement of computational time is highlighted in the introduction and abstract. However, \textcolor{red}{no quantitative comparisons are provided.} I believe the computational time can be added for each method in Table 1. 

Minor suggestions

a- Some recent work on using the complex-valued neural networks (Virtue Patrick et al., arxiv), geometry of deep learning (Golbabaee et al., arxiv)and recurrent neural networks (Oksuz et al.,arxiv) for MRF dictionary matching can be mentioned in the literature review with their strengths and weakneses.
b- Please explain (a.u.) term in Fig.2.
c- Quantitative results can be mentioned in the abstract.
